Moving Towards Open Set Incremental Learning: Readily Discovering New Authors

The classification of textual data often yields important information. Most classifiers work in a closed world setting where the classifier is trained on a known corpus, and then it is tested on unseen examples that belong to one of the classes seen during training. Despite the usefulness of this design, often there is a need to classify unseen examples that do not belong to any of the classes on which the classifier was trained. This paper describes the open set scenario where unseen examples from previously unseen classes are handled while testing. This further examines a process of enhanced open set classification with a deep neural network that discovers new classes by clustering the examples identified as belonging to unknown classes, followed by a process of retraining the classifier with newly recognized classes. Through this process the model moves to an incremental learning model where it continuously finds and learns from novel classes of data that have been identified automatically. This paper also develops a new metric that measures multiple attributes of clustering open set data. Multiple experiments across two author attribution data sets demonstrate the creation an incremental model that produces excellent results.

==> future_work.tex <==
\section{Future Work}
This paper presents an incremental learning approach for NLP. Text based Authorship Attribution can be applied to research involving security and linguistic analysis. Some similar developing work using similar research methods involving image recognition \cite{rebuffi2017icarl}, this can be applied to facial recognition tasks and video surveillance applications. This model can also be further improved by developing a more precise way of distinguishing different pieces of text.

\par
Another method for future research is using backpropagation. Once novel classes are identified, the model should be then able to modify the already trained classifier with the \textit{D\textsubscript{1}} data. Then the model can be tested with the \textit{D\textsubscript{2}} to determine if the model can recognize previously unknown classes. Backpropagation of a neural network requires a fully inter connected set of layers that allow the processing of data through either side of the model \cite{hecht1992theory}. This process would save the step of fully retraining the classifier model. A similar approach to this can also be to add new "neurons" to a deep neural network to allow for an extension of a trained model \cite{draelos2017neurogenesis}.

\begin{comment}
\par
The third piece of new work that can be done is to change the model such that we are not retraining the entire new data set but we are taking the original weights and adding new weights for the identified clustered classes. (Not sure how to do this or how difficult this would be).
\par
The fourth piece of new work that can be done is to attempt to use the Objectosphere approach to identify the novel data samples. This then can be used to compare  results between the Objesctosphere and the Ensemble method. (May take a long time, depends on how the Objectosphere code works)
\end{comment}
